BreakingBED -- Breaking Binary and Efficient Deep Neural Networks by Adversarial Attacks

Deploying convolutional neural networks (CNNs) for embedded applications presents many challenges in balancing resource-efficiency and task-related accuracy. These two aspects have been well-researched in the field of CNN compression. In real-world applications, a third important aspect comes into play, namely the robustness of the CNN. In this paper, we thoroughly study the robustness of uncompressed, distilled, pruned and binarized neural networks against white-box and black-box adversarial attacks (FGSM, PGD, C&W, DeepFool, LocalSearch and GenAttack). These new insights facilitate defensive training schemes or reactive filtering methods, where the attack is detected and the input is discarded and/or cleaned. Experimental results are shown for distilled CNNs, agent-based state-of-the-art pruned models, and binarized neural networks (BNNs) such as XNOR-Net and ABC-Net, trained on CIFAR-10 and ImageNet datasets. We present evaluation methods to simplify the comparison between CNNs under different attack schemes using loss/accuracy levels, stress-strain graphs, box-plots and class activation mapping (CAM). Our analysis reveals susceptible behavior of uncompressed and pruned CNNs against all kinds of attacks. The distilled models exhibit their strength against all white box attacks with an exception of C&W. Furthermore, binary neural networks exhibit resilient behavior compared to their baselines and other compressed variants.

==> backupfiles/final_rebuttal_for_bmvc2020.tex <==
We would like to thank you all for the detailed reviews. We will gladly incorporate your suggestions into the submission. 

Technical Contribution [R1]
BreakingBED shows a new comparison of various adversarial attacks conducted over several variants of compressed CNNs. To the best of our knowledge, such a comprehensive analysis has not yet been carried out. Besides the analytical (i.e. box-plots and PCA) and the visual analysis (CAM), we draw an analogy to the field of mechanics by introducing the stress-strain graphs for robustness evaluation to identify trends (ductile|brittle|strong) among attack/network pairs.

Attack Detection and Defense [R1]
The analysis also helps with pro-active [1] and re-active [2] methods to improve CNN robustness. E.g. we observed ductile-robust models only need to be improved against attacks with high perturbation. These new insights facilitate robust training or reactive filtering methods, where the attack is detected and the input is discarded and/or cleaned. 

[1] Goldblum et al.: Adversarially robust distillation, AAAI, 2020
[2] Papernot et al.: Extending defensive distillation, CoRR, 2017

Analysis Required before Robust Training? [R2]
It is important to understand the robustness potential of the compression techniques before training CNNs against adversarial samples to make them stronger. E.g. our results on KD show inherent robustness compared to the vanilla baseline models. The same effect is amplified after adversarial training [1]. The robustness trends with different pruning regularity (filter|kernel|weight) are also maintained after adversarial training [3].

[3] Ye et al., Adversarial Robustness vs. Model Compression, or Both?, ICCV, 2019

Strength of BNNs or Weakness of GenAttack [R2]
The robustness of BNNs can be attributed to their adversarial strength, as we observe that the GenAttack is capable of breaking other compressed CNNs. This is due to the fact that BNNs require a high amount of perturbation to change a neuron’s firing behavior. This is also observed for LocalSearch. 

CAM Interpretation and Quantitative Analysis  [R2, R3, R4]
We would be happy to open subjective discussions extending the analytical results using the CAM output. The order of the sections 4.1 and 4.2 made our interpretations seem purely subjective. However, we first obtained the data (4.2), then looked at CAM (4.1) to search for correlations that might agree with the results. Nevertheless, correlation is not causation, which makes these CAM results interesting to interpret.

Our interpretations can also be supported using the quantitative analysis as suggested. For an intensity range of (0,255) blue->red, the vanilla and channel pruned models for the car example have the third quartile (Q3) of pixels with an intensity of 114, 96 respectively. When the attack is applied for one iteration, the Q3 value increases (150, 156) indicating the larger ROI. With more iterations, the Q3 value decreases (135, 121).  The pixels above the Q3 indicate reinforced red regions (bonnet) to fool to the nearest class (truck).

Stress Strain Analysis - Analogy [R4]
Indeed not all the concepts from material science are adopted in our analogy and the method can be enhanced. Given the amount of data and points of comparison, we found the proposed stress-strain method helpful in creating a sensible classification of the behaviour of different compressed CNNs under different intensity levels of an attack. We sought to capture definitions for different curvature, steepness and rate of decay with reasonable clarity.

Unify Stress Measurement [R4]
As attack techniques are fundamentally different in their hyper-parameters, this is a difficult (and could be misleading) thing to do.
Instead, it is safer to consider different forms of stress (amplitude, iteration, population-based) as unique ways to break ;) a network, as different forms of mechanical stress (tensile, compressive, shear) exist to deform materials.

==> backupfiles/rebuttal_for_bmvc2020.tex <==
We would like to thank you all for the detailed reviews and the time spent on them. We will gladly incorporate your suggestions into the submission in order to address the weaknesses to the best of our ability.  

\section{Review1:}
%No novelty or technical contribution found
BreakingBED shows a new comparison of various adversarial attacks conducted over several variants of compressed neural networks. To the best of our knowledge, such a comprehensive analysis has not yet been carried out. It allows the direct comparison of neural networks on attacks, in face of the fact that so many hyper-parameters are involved. Besides the analytical comparison (i.e. box plots and the PCA) and the visual analysis (CAM) we draw an analogy to the field of mechanics by introducing the stress-strain graphs for robustness evaluation of CNNs to identify trends (ductile|brittle|strong) among attack/network pairs.
%Suggestion on which compression technique is desirable
The manifold analysis shows that some networks behave in a ductile, brittle or strong manner w.r.t. adversarial attacks. Knowledge about expected attacks or potential compression techniques help the designer or attacker to tackle the associated scenarios. The analysis also helps with pro-active [1] and re-active [2] methods to improve robustness. 
For example, inherently black-box robust neural networks (e.g. BNNs) only need to be further strengthened against white-box attacks. 
Or ductile-robust models only need to be improved against attacks with high perturbation. These new insights facilitate robust training or reactive filtering methods, where the attack is detected and the input is discarded and/or cleaned. This allows the filtering technique to identify and treat an attack only in certain cases, instead of having the effort of anticipating and preempting all possible attacks.

[1] Goldblum et al.: Adversarially robust distillation, AAAI, 2020.
[2] Papernot et al.: Extending defensive distillation, CoRR abs/1705.05264, 2017.

\section{Review2:}
%Different attack types appear to affect different types of compression tech in unique ways.
%Jointly answered in response to Review 1

%Strength of BinaryNets or Weakness of GenAttack
The robustness of BNNs can be attributed to its immanent adversarial strength, as we observe that the GenAttack is capable of breaking other compressed CNNs. This is due to the fact that BNNs require a high amount of perturbation to let a neuron (constrained to +-1) change is fire behavior.
The inherent strength of BNNs can also be observed in other black box attacks such as Local Search. 
%Fig 2 and 3 detail the robustness for BNNs for different kinds of attack schemes (FGSM, PGD, Local Search, GenAttack) indicating its immanent adversarial strength. This also can be observed for local search.

%Analysis required before Robust training?
It is important to understand the robustness potential of the compression techniques before training the CNN against adversarial samples making it stronger. E.g.: Our results on knowledge distillation show inherent robustness compared to the vanilla baseline models. The same effect is amplified after adversarial training [3]. We can also observe the difference in the robustness with varying pruning regularity (filter|kernel|weight). This difference also appears after adversarial training [4].

[3] Goldblum et al. Adversarially Robust Distillation, AAAI, 2020.
[4] Ye et al., Adversarial Robustness vs. Model Compression, or Both?, ICCV, 2019.

%CAM interpretation and Quantitative analysis 
We would like to open a subjective discussions extending the analytical results (Boxplots,PCA,Stress-Strain) using the CAM output. 
%Note to us : Switching the order of the sections 4.1 and 4.2 would make things even clear as our seemingly subjective interpretations were actually done after considering the analytical analysis. 
%Linking phrase missing
There is no mis-prediction in the automobile example image (Tab.1), when the ROI is located at the center (passenger area/cabin). After applying attack, the ROI moves towards the bonnet which is characteristic for classifying a truck. This is observed for several networks. 
%Linking phrase
These interpretations can also be supported using the quantitative analysis as suggested. The vanilla and channel pruned models for the car example exhibit a similar kind of distribution with higher amount of red pixels lying in the third quartile (114, 96). When the attack is applied for one iteration, the third quartile value increases (150, 156) indicating the larger ROI with lower intensity based red regions. When the attack gets more aggressive, the third quartile value decreases (135, 121) indicating reinforced red regions (bonet) to fool w.r.t. next nearest class (truck).  

\section{Review3:}
%Many Results in supplementary material
We fully understand this concern, however, in order to reliably extract trends a large amount of experimentation %(in total over 5500) 
is required. With our proposed analysis techniques (Box-plot, PCA, stress-strain, CAM) we attempted to make sense of the data and draw out useful conclusions and insights for researchers in the field.

%Quantitative analysis 
% For the automobile CAM output without attack (Tab1), the vanilla and pruned models exhibit a similar kind of distribution with higher amount of red pixels lying in the thrid quartile (180.xx, 160.xx), whereas KD and XNOR models demonstrate a focused red region with lower third quartile (130.xx, 90.xx). The same pattern also applied for the cat examples. When the attack is applied for one iteration, the third quartile value decreases for automobile indicating the lower intensity. For cat, the third quartile value increases indicating the reinforcement of the next nearest class.

\section{Review4:}

%Stress Strain Analysis - forced and misleading 
Indeed not all the concepts from material science are adopted in our analogy and the method can be enhanced. Given the amount of data and points of comparison, we found the proposed stress-strain method helpful in creating a sensible classification of the behaviour of different compressed CNNs under different intensity levels of an attack. We hoped to have captured definitions for different curvature, steepness and rate of decay with reasonably clarity.

A "break" in our case is either a network having an accuracy suggesting random guesses or can be application specific. Considering an autonomous car a breaking threshold for an exemplary pedestrian detection is much higher than for a other non critical applications

%Large ROI and Pruning
Jointly answered in response to Review 3

%Merging Stress Strain across attack methods 
As attack techniques are fundamentally different in their hyper-parameters, this is a difficult (and in some cases misleading) thing to do.
Instead, it is safer to consider different forms of stress (amplitude, iteration, population-based) as unique ways to break a network, as different forms of mechanical stress (tensile, compressive, shear) exist to deform materials.

%PCA plots furthermore analysis on robustness
The PCA plots not only explain the correlation between different metrics but also demonstrate the broad ranging white-box robustness irrespective of the compression ratio or normalized compute complexity. Furthermore, large number of data points for binary nets produce higher accuracy after attack indicating its strength against black box attacks.
% Distrubution of the point is more concentrated PCA
% -Discus: +Banana shape, + Curve/Surface 


FINAL CONCLUSIOM: We welcome a discussion on the subjective interpretation of our results, and would like to disclose and discuss it openly with the community  
%backup points
%higher intensity with small ROI - large decision boundary - not easy to change the decision
%                      large ROI - small decision boundary - 
                      
                      
%Regions of interest in CAM output implicitly refers to the area of decision boundary for the corresponding class. Pruning methods try to maintain the prediction accuracy but as consequence weaken the decision boundary [3]. This would result in a larger ROI in the CAM output compared to the vanilla baseline model making them vulnerable to minor perturbations. 
%3. Yazdani et al. The dark side of DNN pruning, ISCA 2018. 
% whereas KD and XNOR models demonstrate a focused red region with lower third quartile (130.xx, 90.xx).
% The same pattern also applied for the cat examples. When the attack is applied for one iteration, the third quartile value decreases for automobile indicating the lower intensity. For cat, the third quartile value increases indicating the reinforcement of the next nearest class.
%
%There is mis-prediction in cat example when the attention of the network starts moving towards cat's snout, classifying as frog. This disturbed attention could be a consequence of either a larger ROI (Tab 1 cat Pruned models) or reinforced focus (binary models mis-classification).  



==> backupfiles/review_from_cvpr2020.tex <==

Reviewer #1
Questions

    1. [Summary] In 3-5 sentences, describe the key ideas, experiments, and their significance.
        This paper presents a comprehensive evaluation of the robustness of efficient neural networks against adversarial perturbation. The authors evaluate several neural network compression and pruning algorithms, such as knowledge distillation, AutoML, XNOR-Net and ABC-Net. The sample attack algorithms include gradient-based attacks: FGSM, PGD, CW, DeepFool, as well as black-box attacks: GenAttack and local search. The authors also propose a metric based on Young's modulus that combines both the adversarial robustness of the model and the attacker's power.
    2. [Strengths] What are the strengths of the paper? Clearly explain why these aspects of the paper are valuable.
        The authors present plenty of experimental results showing that all efficient neural networks are subject to adversarial attack, with some models, such as XNOR-Net, achieving a comparably better robustness. We may be able to derive useful knowledge from these experimental results for strengthening neural networks against adversarial perturbation using compression techniques.
    3. [Weaknesses] What are the weaknesses of the paper? Clearly explain why these aspects of the paper are weak. Please make the comments very concrete based on facts (e.g. list relevant citations if you feel the ideas are not novel).
        1. Although the authors present a thorough evaluation against white-box attacks, the diversity of black-box attacks is lacking. There are many other efficient black-box attacks such as boundary attack (https://arxiv.org/abs/1712.04248), NES attack (https://arxiv.org/abs/1804.08598) and SimBA (https://arxiv.org/abs/1905.07121) that exhibit different behavior.

        2. I find that the sheer quantity of disorganized results is difficult to digest. In particular, I cannot pinpoint a main message of this paper. Are compressed models easier or harder to attack? Are there particular attack strategies that are more suitable. against compressed models? The conclusion that compressed models are vulnerable to adversarial perturbations is of no surprise, and I expect a more non-trivial message even for a survey paper.

        3. The Young's modulus evaluation metric has a critical flaw. The authors propose to compute the ratio between attacker's power (sigma) and model robustness (epsilon). However, the choice of sigma is dependent on the attack algorithm and its various hyperparameters. For example, the number of iterations as a measure of power is highly dependent on the learning rate and optimization algorithm, hence it is impossible to standardize this choice.
    4. [Overall rating] Paper rating
        Weak Reject
    5. [Justification of rating] Please explain how the strengths and weaknesses aforementioned were weighed in for the rating.
        Even as a survey paper, the current draft lacks coherence and a core message for it to be of value. It currently reads as a paper that loosely combines two ideas, adversarial robustness and model compression, without the intricate connections needed for it to fully materialize.

Reviewer #2
Questions

    1. [Summary] In 3-5 sentences, describe the key ideas, experiments, and their significance.
        The paper surveys the effect of adversarial attacks on distilled, pruned and binarized networks. It shows that some compression techniques also induce robustness to adversarial attacks.
    2. [Strengths] What are the strengths of the paper? Clearly explain why these aspects of the paper are valuable.
        + A comprehensive analysis of adversarial robustness on compressed networks, including a large number of experiments with a variety of compression techniques and adversarial attacks.
        + Well written and easy to understand
        + Experiments using CAM show the effect of network compression on the model attention (I would love to see a more comprehensive analysis on this property).
    3. [Weaknesses] What are the weaknesses of the paper? Clearly explain why these aspects of the paper are weak. Please make the comments very concrete based on facts (e.g. list relevant citations if you feel the ideas are not novel).
        - My major concern is that the paper fails to make an overall conclusion. It presents a lot of results and some of them seem to be interesting, but overall it is difficult to get a final impression. For example, an extensive set of performance results is presented in Table 3 - 11 but a detailed analysis is missing. What is the take-home message here?
    4. [Overall rating] Paper rating
        Borderline
    5. [Justification of rating] Please explain how the strengths and weaknesses aforementioned were weighed in for the rating.
        I think the work in this paper is very relevant and interesting, but I think the contribution is limited because it fails to clearly state what insights are to be gained from this large number of experiments. Therefore, I am kind of unsure about the scientific value of the manuscript in its current form.


==> backupfiles/review_wacv.tex <==
Reviewer #2
Questions
1. APPLICATIONS OR ALGORITHMS PAPER? Ideally the authors indicated which track in the CMT version of their title. We'll send an email shortly if not (you probably can't see it otherwise). Note for your evaluation that Applications papers will generally have less in the way of theoretical foundations/approach, more in experimental evaluation. Algorithms papers will be the opposite, more in the theory/approach, perhaps slightly less experiments.
Applications Track
2. PAPER SUMMARY What is the paper about? Please, be concise (2 to 3 sentences).
In this paper, authors provide a analysis on white-box(FGSM, PGD, C&W, Deepfool) and black-box(LocalSearch, GenAttack) adversarial attacks against state-of-the-art vanilla, distilled, pruned and binary neural networks. Detailed experiments and sufficient diagnose are made.
3. PAPER STRENGTHS Please discuss, justifying your comments with the appropriate level of details, the strengths of the paper (i.e. novelty, theoretical approach and/or technical correctness, adequate evaluation, clarity, etc).
1. Authors target on analyzing behaviors of compressed networks, which is valuable and practical.
2. Detailed and sufficient experiments are performed.
3. An efficient evaluation pipeline is proposed.
4. PAPER WEAKNESSES Please discuss, justifying your comments with the appropriate level of details, the weaknesses of the paper (i.e. lack of novelty – given references to prior work-, lack of novelty, technical errors, or/and insufficient evaluation, etc). If you think there is an error in the paper, please explain why it is an error.
1. Important attacking methods are missing. For attacking methods pool, there are no black-box transferable attacking methods. Black-box transferable attacks such as MIFGSM, DIM, TI attack a trained model as surrogate and then transfer to target models. This kind of attacks is significant to black-box studies.
2. Lack of contribution. Although the motivation is valuable and comparison experiments are comprehensive, there is no novel method proposed to improve either attacking or defending performance.
5. FINAL RECOMMENDATION Please use "Borderline" sparingly.
Weak Reject
6. JUSTIFICATION Justify your final recommendation based on the strengths and weaknesses. Please be considerate to the authors and provide constructive feedback.
The motivation is valuable and comparison experiments are comprehensive. It would be a better paper if transferable black-box attacks were considered in experiments. Constructive attacking or defending method is expected to be proposed as well.
Reviewer #3
Questions
1. APPLICATIONS OR ALGORITHMS PAPER? Ideally the authors indicated which track in the CMT version of their title. We'll send an email shortly if not (you probably can't see it otherwise). Note for your evaluation that Applications papers will generally have less in the way of theoretical foundations/approach, more in experimental evaluation. Algorithms papers will be the opposite, more in the theory/approach, perhaps slightly less experiments.
Applications Track
2. PAPER SUMMARY What is the paper about? Please, be concise (2 to 3 sentences).
This paper presents a study on weakness of some forms of CNNs (vanilla, binary, distilled) against white-box and black-box attacks and discuss about individual compression form's performance against each types of adversarial attack.

There's a good intensive coverage on classification task (with CIFAR-10 / ImageNet).
3. PAPER STRENGTHS Please discuss, justifying your comments with the appropriate level of details, the strengths of the paper (i.e. novelty, theoretical approach and/or technical correctness, adequate evaluation, clarity, etc).
The paper was written with good clarity and easy to understand. Experiments were conducted properly with reasonable evaluation mechanism.
4. PAPER WEAKNESSES Please discuss, justifying your comments with the appropriate level of details, the weaknesses of the paper (i.e. lack of novelty – given references to prior work-, lack of novelty, technical errors, or/and insufficient evaluation, etc). If you think there is an error in the paper, please explain why it is an error.
- The evaluation was mainly focused on classification task. There should be some additional experiments on adversarial attacks on different tasks: object recognition / detection, etc.
- When the authors were discussing about CNNs, they simply chose ResNet as the backbone network. One can argue that other complex and SOTA network on public benchmark dataset such as DenseNet, etc can be more robust against these attacks.
- There weren't much discussions on more recent-advanced attack such as GAN-based method, poisoning attack (https://arxiv.org/abs/1804.00792), etc.
5. FINAL RECOMMENDATION Please use "Borderline" sparingly.
Weak Reject
6. JUSTIFICATION Justify your final recommendation based on the strengths and weaknesses. Please be considerate to the authors and provide constructive feedback.
As this is an application-based paper, the analysis should focus into a good representative of CNN architectures, advanced adversarial attacks. This study lacks of breadth coverage (in terms of good coverage of SOTA CNN architecture, adversarial attacks such as GAN-based, tasks-oriented). Therefore, this isn't really a fully comprehensive analysis.

In addition, there has been some recent work on robustness of compression against adversarial attack in both pruning and quantization (ex: https://arxiv.org/abs/1903.12561). I think this should be considered as similar work from this paper, which reduces its novelty.
Reviewer #4
Questions
1. APPLICATIONS OR ALGORITHMS PAPER? Ideally the authors indicated which track in the CMT version of their title. We'll send an email shortly if not (you probably can't see it otherwise). Note for your evaluation that Applications papers will generally have less in the way of theoretical foundations/approach, more in experimental evaluation. Algorithms papers will be the opposite, more in the theory/approach, perhaps slightly less experiments.
Applications Track
2. PAPER SUMMARY What is the paper about? Please, be concise (2 to 3 sentences).
This paper provides an extensive study on the adversarial vulnerability of different variants of CNNs: normal training, distilled, pruned, and binary neural networks. To this end, the authors introduce metrics borrowed from material science, namely stress and strain to present their results.
3. PAPER STRENGTHS Please discuss, justifying your comments with the appropriate level of details, the strengths of the paper (i.e. novelty, theoretical approach and/or technical correctness, adequate evaluation, clarity, etc).
(1) Extensive study over a large variety of adversarial attacks on different network compression methods.
(2) An analogy to stress and strain from material sciences to quantify neural networks into brittle, ductile, and strong networks.
(3) Interesting observations about compressed neural networks, such as the robustness of the XNOR and ABC trained networks to the GenAttack or Localsearch as well as the relatively high robustness of the KD-KL network to a PGD attack.
4. PAPER WEAKNESSES Please discuss, justifying your comments with the appropriate level of details, the weaknesses of the paper (i.e. lack of novelty – given references to prior work-, lack of novelty, technical errors, or/and insufficient evaluation, etc). If you think there is an error in the paper, please explain why it is an error.
Despite the extensive results provided the paper lacks solid new findings or insight into the research of robustness or adversarial examples.
(1) It is already well known that knowledge distillation [10], Pruning [43, 44], and binarization [9] are susceptible to adversarial attacks.
(2) I cannot see the benefit of using “stress” and “strain” over the commonly used adversarial robustness. The authors do not discuss the benefits of introducing new metrics for network robustness (stress and strain). Also, the analogy to material science seems to be misleading. One material is attributed with only one property: brittle, ductile, strong. The results of the authors suggest contradicting properties of models. For example, in Figure 4 the KD-KL network seems to be “strong” under PGD while appearing to be brittle under the GenAttack, DeepFool, etc. Furthermore, the metrics in material sciences are derived from physical properties whereby I am skeptical about such a relationship for DNNs.
(3) I appreciate the extensive experiments, but the authors only hint at some interesting phenomena but do not follow up with possible explanations and supporting experiments/theories. For example: Why do we see an increased FGSM stress on the XNOR-Net in Fig.3a? What is a possible explanation for the boost in robustness when the base CNN is the larger ResNet56 model? What could be the reasons for differing behaviors of binarize ABC models?

[43] Ye, Shaokai, et al. "Adversarial Robustness vs. Model Compression, or Both?." Proceedings of the IEEE/CVF International Conference on Computer Vision. 2019.
[44] Wang, L., Ding, G. W., Huang, R., Cao, Y., & Lui, Y. C. (2018). Adversarial robustness of pruned neural networks.
5. FINAL RECOMMENDATION Please use "Borderline" sparingly.
Weak Reject
6. JUSTIFICATION Justify your final recommendation based on the strengths and weaknesses. Please be considerate to the authors and provide constructive feedback.
Overall the work shows known phenomena and lacks interesting, novel insights into the field of network robustness or adversarial examples.
Reviewer #5
Questions
1. APPLICATIONS OR ALGORITHMS PAPER? Ideally the authors indicated which track in the CMT version of their title. We'll send an email shortly if not (you probably can't see it otherwise). Note for your evaluation that Applications papers will generally have less in the way of theoretical foundations/approach, more in experimental evaluation. Algorithms papers will be the opposite, more in the theory/approach, perhaps slightly less experiments.
Applications Track
2. PAPER SUMMARY What is the paper about? Please, be concise (2 to 3 sentences).
This paper summarized some popular deep neural network compression methods and adversarial methods. Then the author deployed the introduced algorithm to evaluated the robustness.
3. PAPER STRENGTHS Please discuss, justifying your comments with the appropriate level of details, the strengths of the paper (i.e. novelty, theoretical approach and/or technical correctness, adequate evaluation, clarity, etc).
The author demonstrates a good understanding of both compression algorithms and adversarial algorithms. The author gave very sufficient experimental results.
4. PAPER WEAKNESSES Please discuss, justifying your comments with the appropriate level of details, the weaknesses of the paper (i.e. lack of novelty – given references to prior work-, lack of novelty, technical errors, or/and insufficient evaluation, etc). If you think there is an error in the paper, please explain why it is an error.
This paper is lack of novelty. As it is mentioned in the paper, this work is an extensive set of robustness evaluation experiments.
5. FINAL RECOMMENDATION Please use "Borderline" sparingly.
Weak Accept
6. JUSTIFICATION Justify your final recommendation based on the strengths and weaknesses. Please be considerate to the authors and provide constructive feedback.
This paper investigate both of model compresssion and adversarial. Although it is lack of novelty, the experiment results are valuable as a reference for readers.

==> data/30_aa_methods/_JSMA.tex <==
% Jacobian-based Saliency Map Attack (JSMA)

Above\_mentioned methods are all based on generating perturbation with computing the gradient of cost to the whole image. Matrix of perturbation has the the same size as the input image. However not all pixels on image are same important to classifier. Changing only a few pixels can also fool the classifier. Papernot et al. \cite{JSMA} proposed a method to find all sensitive directions based on Jacobian Matrix. This method limits the $l_{0}$ norm of perturbations, which means only a few pixels are perturbed. In each iteration, the gradient of cost on each input image pixel will be provided during the computation. With the Saliency Map method, the importance of each pixel for fooling can be obtained. In our test, we use one-pixel attack, which means only the most important pixel is perturbed with pre-defined strength.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[scale=0.2]{data/Photos/JSMA.png}
%     \caption{Jacobian-based Saliency Map Attack (One-Pixel) \cite{JSMA}}
%     \label{fig:JSMA}
% \end{figure}

==> data/experiments/40_table_comparison.tex <==
Tab.~\ref{tab:FGSMResnet20}-\ref{tab:GenAttackImageNet_eval} cover all the considered white-box (FGSM, PGD, C\&W, DeepFool) and black-box (LocalSearch, GenAttack) attacks on the CIFAR-10-trained ResNet20 compressed variants, as well as ImageNet-trained CNNs. The results for CIFAR-10 ResNet56, for the same experiments are provided in the supplementary material. Tab. ~\ref{tab:FGSMResnet20}-\ref{tab:GenAttackImageNet_eval} provide the accuracy results for the BatchNorm's $\mathtt{statistics}$ mode, while $\mathtt{mini}$-$\mathtt{batch}$ mode results for all the experiments can be found in the supplementary material. $\epsilon$ and $i$ represent the adversarial manipulation budget and iteration count.
For C\&W attacks (Tab.~\ref{tab:CWResnet20_eval}), the target class is $L^{Tar}=deer$ of the CIFAR-10 dataset and $c$ represents the regularization factor in Eq.~\ref{eq:CW}. 
For GenAttacks on CIFAR-10 experiments, the mutation probability $\rho$ and step size $\alpha$ are set to $0.05$ and $1.0$ respectively as demonstrated in ~\cite{GenAttack}. 
%Parent selection probability is based on sampling according to the softmax function applied to the fitness values of the population. 
Elitism is applied for the highest fitness member. On ImageNet experiments $\rho$ and $\alpha$ are adaptive based on the dataset configuration and the population size is 6, as in~\cite{GenAttack}.

==> data/experiments/41_FGSM/410_Experiments_FGSM.tex <==
\noindent
\textbf{Adversarial Attacks on the Fast Gradient Sign Method: }
The experiments examined on FGSM are summarized in Tab.~\ref{tab:FGSMResnet20} for compressed variants of ResNet20 and in Tab.~\ref{tab:FGSMImageNet} for CNNs trained on ImageNet.
Subsequent experiments for all aforementioned adversarial experiments are also examined on ResNet56 and can be found in the supplementary material. The accuracy is given for the BatchNorm's $\mathtt{mini}$-$\mathtt{batch}$ and the $\mathtt{statistics}$ mode after applying the attack. FGSM is applied for the adversarial manipulation budget $\epsilon\in \{2,4,8,16\}$.

==> data/experiments/41_FGSM/411_Experiments_FGSM_eval.tex <==
% \begin{table}[!]
%   \centering
%   \caption{Accuracy (Top1) [\%] of ResNet20/18/50 and its compressed variants after FGSM adversarial attacks.}
%   \resizebox{\columnwidth}{!}{
%   \renewcommand{\arraystretch}{0.95}
%   \begin{tabular}{cl|cccc} 
%     \toprule
%     \textbf{DS}&\textbf{FGSM} & $\epsilon=2$ & $\epsilon=4$ & $\epsilon=8$ & $\epsilon=16$\\
%     \midrule
%     \midrule
%     \multirow{10}{*}{\rotatebox{90}{CIFAR-10}}
%     &\textbf{Vanilla ResNet20}~\cite{He2015DeepRL} (92.46 \%)   &27.21  &16.96  &11.79  &10.04\\
%     &\textbf{KD\_CE}~\cite{contrastive_kd} (92.70 \%)  &26.56  &16.36  &11.73  &9.95\\
%     &\textbf{KD\_KL}~\cite{contrastive_kd}(93.25 \%) &53.01  &43.30  &32.54  &18.69\\
%     &\textbf{AMC(Ch.Prune)}~\cite{AMC2019} (89.76 \%)  &22.31  &12.63  &9.29   &9.50\\
%     &\textbf{AMC(F.Prune)}~\cite{AMC2019} (89.91 \%)  &21.53  &11.69  &8.45   &8.14 \\
%     &\textbf{XNOR}~\cite{rastegari2016} (82.71 \%)  &42.84 &21.71  &8.40    &4.85\\
%     &\textbf{ABC(1$\times$1)}~\cite{lin2017} (83.42 \%)  &38.78  &20.32  &10.93  &6.80\\
%     &\textbf{ABC(3$\times$3)}~\cite{lin2017} (88.94 \%) &41.98  &22.99  &13.20  &9.62\\
%     &\textbf{ABC(5$\times$5)}~\cite{lin2017} (90.64 \%)&38.70  &24.18  &17.78  &13.86\\
%     &\textbf{ABC(7$\times$7)}~\cite{lin2017} (91.34 \%) &40.11  &27.45  &20.94  &16.61\\
%     \midrule
%     \multirow{6}{*}{\rotatebox{90}{ImageNet}}
%     &\textbf{ResNet50}~\cite{He2015DeepRL} (75.43 \%)    &22.18&16.24&12.08&7.46\\
%     \cmidrule{2-6}
%     &\textbf{Vanilla ResNet18}~\cite{He2015DeepRL} (69.00 \%)   &12.82  &8.16   &5.19   &2.95\\
%     &\textbf{AMC(Ch.Prune)}~\cite{AMC2019} (67.62 \%)   &11.18  &6.64   &3.99   &2.34\\
%     &\textbf{XNOR}~\cite{rastegari2016} (49.10 \%)       &7.57   &4.54   &2.19   &0.93\\
%     &\textbf{ABC(1$\times$1)}~\cite{lin2017} (51.07 \%) &9.11&4.65&2.30&1.13\\
%     &\textbf{ABC(3$\times$3)}~\cite{lin2017} (59.83 \%) &11.33&5.73&2.65&1.43\\
%     \bottomrule 
%     \end{tabular}}
%   \label{tab:FGSMResnet20}
% \end{table}

==> data/experiments/41_FGSM/413_Experiments_FGSM_ImageNet_eval.tex <==
% \begin{table}[!]
%   \centering
%   \caption{FGSM attacks for CNNs trained on ImageNet.}
%   \resizebox{\columnwidth}{!}{
%   \renewcommand{\arraystretch}{0.9}
%   \begin{tabular}{l|cccc} 
%     \toprule
%     \textbf{FGSM}  &$\epsilon=2$ & $\epsilon=4$ & $\epsilon=8$ & $\epsilon=16$\\
%     \midrule
%     \midrule
%     \textbf{ResNet50}~\cite{He2015DeepRL} (75.43 \%)    &22.18&16.24&12.08&7.46\\    
%     \textbf{ResNet18}~\cite{He2015DeepRL} (69.00 \%)   &12.82  &8.16   &5.19   &2.95\\
%     \textbf{AMC(Ch.Prune)}~\cite{AMC2019} (67.62 \%)   &11.18  &6.64   &3.99   &2.34\\
%     \textbf{XNOR}~\cite{rastegari2016} (49.10 \%)       &7.57   &4.54   &2.19   &0.93\\
%     \textbf{ABC(1$\times$1)}~\cite{lin2017} (51.07 \%) &9.11&4.65&2.30&1.13\\
%     \textbf{ABC(3$\times$3)}~\cite{lin2017} (59.83 \%) &11.33&5.73&2.65&1.43\\
%     \bottomrule                                
%     \end{tabular}}
%   \label{tab:FGSMImageNet}
% \end{table}



==> data/experiments/42_PGD/420_Experiments_PGD.tex <==
\noindent
\textbf{Adversarial Attacks on Projected Gradient Descent: }
The adversarial attacks examined w.r.t. PGD are summarized in Tab.~\ref{tab:PGDResnet20_eval} and \ref{tab:PGDImageNet_eval} for the BatchNorm's $\mathtt{statistics}$ mode respectively. 
the accuracy of the respective CNNs after the attack for the BatchNorm's $\mathtt{mini}$-$\mathtt{batch}$ mode are detailed in the supplementary material.
PGD is applied for $\epsilon\in \{0.1,0.5,1.0,2.0\}$ multiple iterations $i\in\{2,3,4,5\}$

==> data/experiments/43_CW/430_Experiments_CW.tex <==
\noindent
\textbf{Adversarial Attacks on Carlini \& Wagner: }
The adversarial attacks examined w.r.t. C\&W are summarized in Tab.~\ref{tab:CWResnet20_eval} for the BatchNorm's $\mathtt{statistics}$ mode respectively. It should be noted that results for ResNet56 are detailed in the supplementary material.
The regularization factor is $c\in\{0.01,0.1,1.0,5.0,10.0\}$ and the attack is run for $i\in\{1,10,20,50\}$ iterations for the target class $L^{Tar}=deer$ of the CIFAR-10 dataset.

==> data/experiments/44_DeepFool/441_Experiments_Deepfool_ResNet20_eval.tex <==
\begin{table}[!]
  \centering
  \resizebox{0.7\textwidth}{!}{
  \renewcommand{\arraystretch}{0.9}
  \begin{tabular}{l|cccc} 
    \toprule
    \textbf{DeepFool} &$i=1$  &$i=5$ &$i=10$ &$i=20$\\
    \midrule
    \midrule
    \textbf{Vanilla}~\cite{He2015DeepRL} (92.46 \%) &37.75	&5.15	&5.11	&5.09\\%37.75  &5.15   &5.12   &5.09 \\
    \textbf{KD-CE}~\cite{contrastive_kd} (92.70 \%)  &38.10	&4.78	&4.75	&4.80\\%38.10  &4.78   &4.75   &4.79 \\
    \textbf{KD-KL}~\cite{contrastive_kd} (93.25 \%)&61.28	&6.35	&4.64	&4.53\\%60.72  &6.24   &4.79   &4.72 \\
    \textbf{Ch.Prune}~\cite{AMC2019} (89.76 \%)    &33.18	&6.79	&6.74	&6.66\\%33.18  &6.79   &6.74   &6.68 \\
    \textbf{F.Prune}~\cite{AMC2019} (89.91 \%)     &32.23	&6.39	&6.27	&6.25\\
    \textbf{XNOR}~\cite{rastegari2016} (82.71 \%)  &62.59	&15.51	&11.38	&10.40\\%62.59  &15.49  &11.39  &10.40 \\
    \textbf{ABC(1$\times$1)}~\cite{lin2017} (83.42 \%)&57.17	&13.00	&10.59	&9.77\\%57.16  &12.99  &10.58  &9.77 \\
    \textbf{ABC(3$\times$3)}~\cite{lin2017} (88.94 \%) &55.98	&9.60	&7.73	&7.39\\%55.98  &9.59   &7.73   &7.39 \\
    \textbf{ABC(5$\times$5)}~\cite{lin2017} (90.64 \%) &51.10	&7.96	&6.99	&6.80\\%51.09  &7.96   &6.99   &6.78 \\
    \textbf{ABC(7$\times$7)}~\cite{lin2017} (91.34 \%)&48.26	&6.96	&6.39	&6.31\\%48.26  &6.96   &6.39   &6.31 \\
    \bottomrule                                
    \end{tabular}}
    \vspace{1em}
    \caption{Accuracy (Top1) [\%] of ResNet20 like CNNs after DeepFool adversarial attacks for CIFAR-10.}
  \label{tab:DeepFoolResnet20}
\end{table}


==> data/experiments/45_LocalSearch/450_Experiments_LocalSearch.tex <==
\noindent
\textbf{Adversarial Attacks on LocalSearch: }
Tab.~\ref{tab:LocalSearchResNet20_eval} shows the accuracy of compressed versions of ResNet20 when attacked by LocalSearch. The attack is run for $i\in\{50,100,150,200\}$ iterations respectively.

==> data/experiments/46_GenAttack/460_Experimental_Setup_GenAttack.tex <==
\noindent
\textbf{Adversarial Attacks on GenAttack: }
The GenAttack is compared by performing experiments on different CNN models on CIFAR-10 and ImageNet datasets. For the CNN models trained on CIFAR-10 dataset, we choose the number of iterations $i$ as 200. the mutation probability $\rho$ and step size $\alpha$ are set to $5e-2$ and $1.0$ respectively as demonstrated in ~\cite{GenAttack}. Parent selection probability is based on sampling according to the softmax function applied to the fitness values of the population. Elitism is applied for the highest fitness member. On ImageNet experiments $\rho$ and $\alpha$ are adaptive based on the dataset configuration and the population size is fixed to 6, as in~\cite{GenAttack}. The experiments for all the models are performed with the strengths $\epsilon$ = 6, 16.\nael{strengths are 8 and 12 in table \ref{tab:GenAttack_ResNet20_eval}, and pop is 6 or 16. Which one is the typo, the text or the table?}

==> data/experiments/47_CAM/471_CAM_ResNet20.tex <==
\begin{table}[!]
\centering
\caption{CAM for ResNet20 and it's compressed variants performed on non attacked and DeepFool attacked images.}
\setlength{\tabcolsep}{1pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&No AA & \multicolumn{2}{c}{DeepFool\cite{Deepfool}}&No AA&\multicolumn{2}{c}{DeepFool\cite{Deepfool}} \\
&$L$=$Car$&$i$=$1$&$i$=$5$&$L$=$Cat$&$i$=$1$&$i$=$5$\\
\midrule
\midrule
%auto
\adjustbox{valign=t}{\makecell[l]{\textbf{Image}\\$I \rightarrow$ \fcolorbox{red}{white}{$I^{Adv}$}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_raw_image_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/i1_ResNet20_Vanilla_adv_image_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/i5_ResNet20_Vanilla_adv_image_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_raw_image_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/i1_ResNet20_Vanilla_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/i5_ResNet20_Vanilla_adv_image_103.png}}}\\
%Vanilla
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet20}~\cite{He2015DeepRL}\\(92.46 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_overlay_103.png}}}\\
%KD_CE
\adjustbox{valign=t}{\makecell[l]{\textbf{KD\_CE}~\cite{contrastive_kd}\\(92.70 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_KD_CE_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_KD_CE_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_KD_CE_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_KD_CE_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_KD_CE_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_KD_CE_overlay_103.png}}}\\
%KD_KL
\adjustbox{valign=t}{\makecell[l]{\textbf{KD\_KL}~\cite{contrastive_kd}\\(93.25 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_KD_KL_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_KD_KL_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_KD_KL_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_KD_KL_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_KD_KL_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_KD_KL_overlay_103.png}}}\\
%AMC
\adjustbox{valign=t}{\makecell[l]{\textbf{AMC(Ch.Prune)}~\cite{AMC2019}\\(89.76 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_AMC_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_AMC_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_AMC_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_AMC_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_KD_KL_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_KD_KL_overlay_103.png}}}\\
%XNOR
\adjustbox{valign=t}{\makecell[l]{\textbf{XNOR}~\cite{rastegari2016}\\(82.71 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_XNOR_overlay_1604.png}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_XNOR_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_XNOR_overlay_103.png}}}\\
%ABC1x1
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(1$\times$1)}~\cite{lin2017}\\(83.42 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_ABC1x1_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_ABC1x1_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_ABC1x1_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_ABC1x1_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_ABC1x1_overlay_103.png}}}\\
%ABC3x3
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(3$\times$3)}~\cite{lin2017}\\(88.94 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_ABC3x3_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_ABC3x3_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_ABC3x3_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_ABC3x3_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_ABC1x1_overlay_103.png}}}\\
%ABC5x5
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(5$\times$5)}~\cite{lin2017}\\(90.64 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_ABC5x5_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_ABC5x5_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_ABC5x5_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_ABC5x5_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_ABC5x5_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_ABC5x5_overlay_103.png}}}\\
%ABC7x7
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(7$\times$7)}~\cite{lin2017}\\(91.34 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/auto/ResNet20_ABC7x7_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i1/ResNet20_ABC7x7_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_auto_i5/ResNet20_ABC7x7_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/cat/ResNet20_ABC7x7_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i1/ResNet20_ABC7x7_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet20/aa_cat_i5/ResNet20_ABC7x7_overlay_103.png}}}\\
\bottomrule
\end{tabular}}
\label{tab:cam_resnet20}
\vspace{-3ex}
\end{table}

==> data/experiments/47_CAM/472_CAM_ResNet56.tex <==
\begin{table}[!]
\centering
\caption{CAM for ResNet56 and it's compressed variants performed on non attacked and DeepFool attacked images.}
\setlength{\tabcolsep}{1pt}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&No AA & \multicolumn{2}{c}{DeepFool\cite{Deepfool}}&No AA&\multicolumn{2}{c}{DeepFool\cite{Deepfool}} \\
&$L$=$Car$&$i$=$5$&$i$=$10$&$L$=$Cat$&$i$=$1$&$i$=$5$\\
\midrule
\midrule
%auto
\adjustbox{valign=t}{\makecell[l]{\textbf{Image}\\$I \rightarrow$ \fcolorbox{red}{white}{$I^{Adv}$}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_raw_image_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/i5_ResNet56_adv_image_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/i10_ResNet56_adv_image_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_raw_image_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/i1_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/i5_ResNet56_adv_image_103.png}}}\\
%Vanilla
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet56}~\cite{He2015DeepRL}\\(93.88 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_overlay_103.png}}}\\
%AMC
\adjustbox{valign=t}{\makecell[l]{\textbf{AMC(Ch.Prune)}~\cite{AMC2019}\\(92.86 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_AMC_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_overlay_103.png}}}\\
%XNOR
\adjustbox{valign=t}{\makecell[l]{\textbf{XNOR}~\cite{rastegari2016}\\(83.24 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_XNOR_overlay_1604.png}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_XNOR_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_XNOR_overlay_103.png}}}\\
%ABC(1x1)
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(1$\times$1)~\cite{lin2017}}\\(86.29 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC1x1_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC1x1_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_ABC1x1_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC1x1_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC1x1_overlay_103.png}}}\\
%ABC(3x3)
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(3$\times$3)~\cite{lin2017}}\\(92.48 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC3x3_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC3x3_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_ABC3x3_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC3x3_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC3x3_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC3x3_overlay_103.png}}}\\
%ABC(5x5)
\adjustbox{valign=t}{\makecell[l]{\textbf{ABC(5$\times$5)~\cite{lin2017}}\\(92.82 \%)}}&
%auto
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC5x5_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC5x5_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i10/ResNet56_ABC5x5_overlay_1604.png}}}&
%cat
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC5x5_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC5x5_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC5x5_overlay_103.png}}}\\
\bottomrule
\end{tabular}}
\label{tab:cam_resnet56}
\vspace{-3ex}
\end{table}

==> data/experiments/47_CAM/472_CAM_ResNet56_bmvc.tex <==
\begin{table}[ht]
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|c|c|cccc|cccc}
\toprule
&&\multicolumn{1}{c|}{\textbf{Vanilla}}&\multicolumn{1}{c|}{\textbf{Distilled}}&\multicolumn{4}{c|}{\textbf{Pruned}}&\multicolumn{4}{c}{\textbf{Binary}}\\
%\multirow{2}{*}{\textbf{Model}}&No AA & \multicolumn{2}{c}{DeepFool\cite{Deepfool}}&No AA&\multicolumn{2}{c}{DeepFool\cite{Deepfool}} \\
%&$L$=$Car$&$i$=$1$&$i$=$5$&$L$=$Cat$&$i$=$1$&$i$=$5$\\
%\textbf{DeepFool}
\multicolumn{2}{c|}{\textbf{Image$\rightarrow$ \fcolorbox{red}{white}{$I^{Adv}$}}}&
ResNet56&
%\textbf{KD\_CE}&
KD-KL&
Channel&
Filter&
Kernel&
Weight&
XNOR&
ABC(1$\times$1)&
ABC(3$\times$3)&
ABC(5$\times$5)\\
&&(93.88 \%)&
(94.24 \%)&
(92.86 \%)&
(92.86\%)&
(93.09\%)&
(93.04\%)&
(93.54\%)&
(83.24 \%)&
(86.29 \%)&
(92.48 \%)\\
\midrule
\midrule
%\multirow{1}{*}{\rotatebox[origin=c]{90}{\makecell[c]{No AA}}}&
\adjustbox{valign=t}{\rotatebox{90}{\makecell{No AA}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_raw_image_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_overlay_1604.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_KD_CE_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_KD_KL_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_channel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_filter_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_kernel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_weight_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC1x1_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC3x3_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC5x5_overlay_1604.png}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC7x7_overlay_1604.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=1$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/i1_adv_image_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_overlay_1604.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_KD_CE_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_KD_KL_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_channel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_filter_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_kernel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_weight_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_XNOR_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC1x1_overlay_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC3x3_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC5x5_overlay_1604.png}}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC7x7_overlay_1604.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=5$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/i5_adv_image_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_overlay_1604.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_KD_CE_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_KD_KL_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_channel_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_filter_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_kernel_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_weight_prune_overlay_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_XNOR_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC1x1_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC3x3_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC5x5_overlay_1604.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC7x7_overlay_1604.png}}}\\
\midrule
\adjustbox{valign=t}{\rotatebox{90}{\makecell{No AA}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_raw_image_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_overlay_103.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_KD_CE_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_KD_KL_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_channel_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_filter_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_kernel_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_weight_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_XNOR_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC1x1_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC3x3_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC5x5_overlay_103.png}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC7x7_overlay_103.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=1$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/i1_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_overlay_103.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_KD_CE_overlay_103.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_KD_KL_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_channel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_filter_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_kernel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_weight_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC3x3_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC5x5_overlay_103.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC7x7_overlay_103.png}}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=5$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/i5_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_overlay_103.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_KD_CE_overlay_103.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_KD_KL_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_channel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_filter_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_kernel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_weight_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC3x3_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC5x5_overlay_103.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC7x7_overlay_103.png}}}\\
\bottomrule
\end{tabular}}
\vspace{-1ex}
\caption{CAM for ResNet56 and its compressed variants performed on non-attacked and DeepFool attacked images on CIFAR-10 dataset}
\vspace{-3ex}
\label{tab:cam_resnet56}
\end{table}

==> data/experiments/47_CAM/472_CAM_ResNet56_wacv.tex <==
\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|c|c|cccc|cccc}
\toprule
&&\multicolumn{1}{c|}{\textbf{Vanilla}}&\multicolumn{1}{c|}{\textbf{Distilled}}&\multicolumn{4}{c|}{\textbf{Pruned}}&\multicolumn{4}{c}{\textbf{Binary}}\\
%\multirow{2}{*}{\textbf{Model}}&No AA & \multicolumn{2}{c}{DeepFool\cite{Deepfool}}&No AA&\multicolumn{2}{c}{DeepFool\cite{Deepfool}} \\
%&$L$=$Car$&$i$=$1$&$i$=$5$&$L$=$Cat$&$i$=$1$&$i$=$5$\\
%\textbf{DeepFool}
\multicolumn{2}{c|}{\textbf{Image$\rightarrow$ \fcolorbox{red}{white}{$I^{Adv}$}}}&
ResNet56&
%\textbf{KD\_CE}&
KD-KL&
Channel&
Filter&
Kernel&
Weight&
XNOR&
ABC(1$\times$1)&
ABC(3$\times$3)&
ABC(5$\times$5)\\
&&(93.88 \%)&
(94.24 \%)&
(92.86 \%)&
(92.86\%)&
(93.09\%)&
(93.04\%)&
(93.54\%)&
(83.24 \%)&
(86.29 \%)&
(92.48 \%)\\
\midrule
\midrule
%\multirow{1}{*}{\rotatebox[origin=c]{90}{\makecell[c]{No AA}}}&
\adjustbox{valign=t}{\rotatebox{90}{\makecell{No AA}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_raw_image_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_overlay_1604.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_KD_CE_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_KD_KL_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_channel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_filter_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_kernel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_AMC_weight_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_XNOR_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC1x1_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC3x3_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC5x5_overlay_1604.png}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/auto/ResNet56_ABC7x7_overlay_1604.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=1$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/i1_adv_image_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_overlay_1604.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_KD_CE_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_KD_KL_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_channel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_filter_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_kernel_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_AMC_weight_prune_overlay_1604.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_XNOR_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC1x1_overlay_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC3x3_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC5x5_overlay_1604.png}}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i1/ResNet56_ABC7x7_overlay_1604.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=5$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/i5_adv_image_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_overlay_1604.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_KD_CE_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_KD_KL_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_channel_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_filter_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_kernel_prune_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_AMC_weight_prune_overlay_1604.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_XNOR_overlay_1604.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC1x1_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC3x3_overlay_1604.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC5x5_overlay_1604.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_auto_i5/ResNet56_ABC7x7_overlay_1604.png}}}\\
\midrule
\adjustbox{valign=t}{\rotatebox{90}{\makecell{No AA}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_raw_image_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_overlay_103.png}}&
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_KD_CE_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_KD_KL_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_channel_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_filter_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_kernel_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_AMC_weight_prune_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_XNOR_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC1x1_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC3x3_overlay_103.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC5x5_overlay_103.png}}\\
%\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/cat/ResNet56_ABC7x7_overlay_103.png}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=1$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/i1_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_overlay_103.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_KD_CE_overlay_103.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_KD_KL_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_channel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_filter_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_kernel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_AMC_weight_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC3x3_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC5x5_overlay_103.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i1/ResNet56_ABC7x7_overlay_103.png}}}\\
\adjustbox{valign=t}{\rotatebox{90}{\makecell{$i=5$}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/i5_adv_image_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_overlay_103.png}}}&
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_KD_CE_overlay_103.png}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_KD_KL_overlay_103.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_channel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_filter_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_kernel_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_AMC_weight_prune_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_XNOR_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC1x1_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC3x3_overlay_103.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC5x5_overlay_103.png}}}\\
%\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ResNet56/aa_cat_i5/ResNet56_ABC7x7_overlay_103.png}}}\\
\bottomrule
\end{tabular}}
\vspace{-1ex}
\caption{CAM for ResNet56 and its compressed variants performed on non-attacked and DeepFool attacked images on CIFAR-10 dataset \manoj{Can we consider removing the CAT based CAM images, so that we have no confusion in interpretation?}}
\vspace{-3ex}
\label{tab:cam_resnet56}
\end{table*}

==> data/experiments/47_CAM/473_CAM_ImageNet.tex <==
\begin{table}[!]
\centering
\caption{CAM for CNNs trained on ImageNet performed on non attacked and PGD attacked images.}
\setlength{\tabcolsep}{1pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&No AA & \multicolumn{3}{c}{PGD\cite{}}\\
&$L$=$race car$ &$i=1$ & $i=2$ &  $i=4$ \\
\midrule
\midrule
%auto
\adjustbox{valign=t}{\makecell[l]{\textbf{Image}\\$I\rightarrow$ \fcolorbox{red}{white}{$I^{Adv}$}}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/racecar/ResNet18_raw_image_28.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i1/ResNet18_raw_image_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i2/ResNet18_raw_image_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i4/ResNet18_raw_image_28.png}}}\\
%ResNet50 Vanilla
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet50}~\cite{He2015DeepRL}\\(75.43\%)}}&
%racecar
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/racecar/ResNet50_overlay_28.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i1/ResNet50_overlay_28.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i2/ResNet50_overlay_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i4/ResNet50_overlay_28.png}}}\\
%Vanilla
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet18}~\cite{He2015DeepRL}\\(69.00\%)}}&
%racecar
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/racecar/ResNet18_overlay_28.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i1/ResNet18_overlay_28.png}}&
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i2/ResNet18_overlay_28.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i4/ResNet18_overlay_28.png}}}\\
%ResNet18 AMC
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet18-AMC}\\\textbf{(Ch.Prune)}\cite{AMC2019} \\(67.62\%)}}&
%racecar
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/racecar/ResNet18_AMC_overlay_28.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i1/ResNet18_AMC_overlay_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i2/ResNet18_AMC_overlay_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i4/ResNet18_AMC_overlay_28.png}}}\\
%ResNet18 XNOR
\adjustbox{valign=t}{\makecell[l]{\textbf{ResNet18-XNOR}~\cite{rastegari2016}\\(49.10\%)}}&
%racecar
\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/racecar/ResNet18_XNOR_overlay_28.png}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i1/ResNet18_XNOR_overlay_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i2/ResNet18_XNOR_overlay_28.png}}}&
\fcolorbox{red}{red}{\adjustbox{valign=t}{\includegraphics[width=0.15\columnwidth]{img/CAM_ImageNet/aa_racecar_i4/ResNet18_XNOR_overlay_28.png}}}\\
\bottomrule
\end{tabular}}
\label{tab:cam_imagenet}

\end{table}

==> img/data_mining/blackbox_data/tikz_plot_blackbox_pca.tex <==



%-2.003,-2.365,Attack acc
%0,0,
%2.7107,-0.6238,Size
%0,0,
%2.571,-0.992,NCC
%0,0,
%2.632,-1.004,Acc
%0,0,
%0.4075,4.045,Norm AAS
%0,0,

\definecolor{happi_blue}{rgb}{0.141, 0.443, 0.639} 
\definecolor{happi_yellow}{rgb}{1, 0.764, 0 }
\definecolor{happi_red}{rgb}{ 1, 0.341, 0.2 }

\begin{tikzpicture}
\begin{axis}[
    height=0.25\textwidth,
    width=0.5\textwidth,
    grid=major, 
    grid style={dashed,gray!30},
    legend pos=south west,
    xlabel=Factor1 (59.46\%), 
    ylabel=Factor2 (25.43\%),
    xticklabel style = {font=\tiny},
    yticklabel style = {font=\tiny, rotate=90, yshift=-0.3ex},
    ylabel style = {font=\tiny, yshift=-5.75ex},
	xlabel style = {font=\tiny, yshift=2ex},
    xmin=-4,
    xmax=3,
    ymin=-3,
    ymax=5,
    cycle list name=mycolorlist2]
    
    \addplot table[x=f1_vanilla, y=f2_vanilla, col sep=comma] {data_to_plot.csv};
    
    
    \addplot table[x=f1_chpr, y=f2_chpr, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_fpr, y=f2_fpr, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_kpr, y=f2_kpr, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_wpr, y=f2_wpr, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_xnor, y=f2_xnor, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_abc1, y=f2_abc1, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_abc3, y=f2_abc3, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_abc5, y=f2_abc5, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_kdce, y=f2_kdce, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_kdkl, y=f2_kdkl, col sep=comma] {data_to_plot.csv};

    \addlegendentry{Vanilla};
    \addlegendentry{AMC-CH};
    \addlegendentry{AMC-F};
    \addlegendentry{AMC-K};
    \addlegendentry{AMC-W};
    \addlegendentry{XNOR};
    \addlegendentry{ABC($1\times1$)};
    \addlegendentry{ABC($3\times3$)};
    \addlegendentry{ABC($5\times5$)};
    \addlegendentry{KD-CE};
    \addlegendentry{KD-KL};
	\legend{};
	\node[align=left, anchor=west] (N) at (axis cs: -2.003,-2.365) {\tiny Acc. after Attack};
	\draw[->] (axis cs: 0,0) -- (axis cs: -2.003,-2.365);
	
	\node[align=center, text width=2cm, anchor=south] (N) at (axis cs: 2.6107,-0.9838) {\tiny Memory};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.7107,-0.6238);
	
	\node[align=center, text width=2cm, anchor=north] (N) at (axis cs: 2.632,-1) {\tiny NCC};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.571,-0.992);
	
	\node[align=center, text width=2cm, anchor=north] (N) at (axis cs: 2.771,-0.5) {\tiny Acc};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.632,-1.004);
	
	\node[align=left, text width=2cm, anchor=west] (N) at (axis cs: 0.4075,4.045) {\tiny Norm AAS};
	\draw[->] (axis cs: 0,0) -- (axis cs: 0.4075,4.045);
\end{axis}
\end{tikzpicture}

==> img/data_mining/plot_legend_PCA.tex <==
\begin{tikzpicture}	
	\begin{axis}[
		name=legend,
		width=\textwidth,
		height=3ex,
		hide axis,
        legend style={at={(0.1,0)},anchor=west, legend columns=-1, draw = none, nodes={scale=0.5, transform shape}, column sep=2pt},
		ymin=0,
        ymax=1,
        xmin=0,
        xmax=1,
		]
		\addlegendimage{Pal_1, mark=x,mark options={scale=1}, line width=1pt, only marks}
       	\addlegendentry{Vanilla};
       	\addlegendimage{Pal_2, mark=square,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{Ch.Prune};
		\addlegendimage{Pal_7, mark=square,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{F.Prune};
		\addlegendimage{Pal_6,mark=square,mark options={scale=1}, line width=1pt, only marks}
        \addlegendentry{K.Prune};
        \addlegendimage{Pal_3,mark=square,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{W.Prune};
		\addlegendimage{Pal_4, mark=diamond,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{XNOR};
		\addlegendimage{Pal_5, mark=triangle,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{ABC($1\times1$)};
		\addlegendimage{Pal_6,mark=triangle,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{ABC($3\times3$)};
		\addlegendimage{Pal_8,mark=triangle,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{ABC($5\times5$)};
        \addlegendimage{Pal_1 ,mark=o,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{KD-CE};
		\addlegendimage{Pal_2,mark=o,mark options={scale=1}, line width=1pt, only marks}
		\addlegendentry{KD-KL};
	\end{axis}
\end{tikzpicture}

==> img/data_mining/whitebox_data/tikz_plot_whitebox_pca.tex <==



% 0.27961568,-2.95887969,Attack acc
% 0,0,
% 2.5036876,-0.07592863,Size
% 0,0,
% 2.5104,0.062721,NCC
% 0,0,
% 2.28758,0.2892,Acc
% 0,0,
% -0.0805,2.9719,Norm AAS
% 0,0,

\definecolor{happi_blue}{rgb}{0.141, 0.443, 0.639} 
\definecolor{happi_yellow}{rgb}{1, 0.764, 0 }
\definecolor{happi_red}{rgb}{ 1, 0.341, 0.2 }

\begin{tikzpicture}
\begin{axis}[
    height=0.25\textwidth,
    width=0.5\textwidth,
    grid=major, 
    grid style={dashed,gray!30},
    legend pos=south west,
    xlabel=Factor1 (52.07\%), 
    ylabel=Factor2 (29.20\%),
    xticklabel style = {font=\tiny},
    yticklabel style = {font=\tiny, rotate=90, yshift=-0.3ex},
    ylabel style = {font=\tiny, yshift=-5.75ex},
	xlabel style = {font=\tiny, yshift=2ex},
    xmin=-4,
    xmax=3,
    ymin=-4,
    ymax=4,
    cycle list name=mycolorlist2]
    
    \addplot table[x=f1_vanilla, y=f2_vanilla, col sep=comma] {data_to_plot.csv};
    
    
    \addplot table[x=f1_chpr, y=f2_chpr, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_fpr, y=f2_fpr, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_kpr, y=f2_kpr, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_wpr, y=f2_wpr, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_xnor, y=f2_xnor, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_abc1, y=f2_abc1, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_abc3, y=f2_abc3, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_abc5, y=f2_abc5, col sep=comma] {data_to_plot.csv};
    
    \addplot table[x=f1_kdce, y=f2_kdce, col sep=comma] {data_to_plot.csv};
    \addplot table[x=f1_kdkl, y=f2_kdkl, col sep=comma] {data_to_plot.csv};

    \addlegendentry{Vanilla};
    \addlegendentry{AMC-CH};
    \addlegendentry{AMC-F};
    \addlegendentry{AMC-K};
    \addlegendentry{AMC-W};
    \addlegendentry{XNOR};
    \addlegendentry{ABC($1\times1$)};
    \addlegendentry{ABC($3\times3$)};
    \addlegendentry{ABC($5\times5$)};
    \addlegendentry{KD-CE};
    \addlegendentry{KD-KL};
	\legend{};
	\node[align=left, anchor=west] (N) at (axis cs: 0.27961568,-2.9887969) {\tiny Acc. after Attack};
	\draw[->] (axis cs: 0,0) -- (axis cs: 0.27961568,-2.95887969);
	
	\node[align=left, text width=2cm, anchor=west] (N) at (axis cs: 2.0036876,-0.3892863) {\tiny Memory};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.5036876,-0.07592863);
	
	\node[align=left, text width=2cm, anchor=west] (N) at (axis cs: 2.4104,0.062721) {\tiny NCC};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.5104,0.062721);
	
	\node[align=left, text width=2cm, anchor=west] (N) at (axis cs: 2.18758,0.7092) {\tiny Acc};
	\draw[->] (axis cs: 0,0) -- (axis cs: 2.28758,0.3092);
	
	\node[align=left, text width=2cm, anchor=west] (N) at (axis cs: -0.2,3.5719) {\tiny Norm AAS};
	\draw[->] (axis cs: 0,0) -- (axis cs: -0.0805,2.9719);
\end{axis}
\end{tikzpicture}

==> misc/todoes.tex <==
\begin{todolist}
%\item[\done] test
\item Make all Models available in the ModelZoo ():
\begin{todolist}
\item[\done] ResNet20 - Acc. 92.47
\item[\done] ResNet20 KD ce\_loss - Acc. 92.70
\item[\done] ResNet20 KD kl\_divergence (temp:20!!) - Acc. 93.25
\item[\done] ResNet20 XNOR - Acc. 82.95
\item[\done] ResNet20 ABC(1x1) - Acc: 83.59
\item[\done] ResNet20 ABC(3x3) - Acc: 88.90
\item[\done] ResNet20 ABC(5x5) - Acc: 90.33
\item[\done] ResNet20 ABC(7x7) - Acc: 91.22
\item[\done] ResNet20 AMC Pruned - \\ Acc. 89.76 (channel) \\ Acc. 89.92 (filter)\manoj{verify!}\qi{YUankai has modified amc for filter prune}
\item[\done] ResNet56 - Acc. 93.88
\item[\done] ResNet56 XNOR - 83.27
\item[\done] ResNet56 ABC(1x1) - 86.25
\item[\done] ResNet56 ABC(3x3) - Acc: 92.09
\item[\done] ResNet56 ABC(5x5) - Acc: 92.72
\item[\done] ResNet56 AMC Pruned - Acc. 92.86 (Channel\_Prune HW\_constraint) \\ - Acc. 93.08 (Filter\_Prune HW\_constraint)
\item[\done] ResNet18 - Acc. 69.89
\item[\done] ResNet18 XNOR - 47.19 (XNOR paper: 51.2)
\item ResNet18 AMC \alex{does qi has snapshot.} \qi{Not yet, however there is no Config file for ResNet18 ImageNet in ModelZoo.}
\item ResNet34 - \alex{recover snapshot}


\item MobileNetV2 -  \alex{recover snapshot} \yuankai{Acc. 66.56 fine tuning...}
\end{todolist}
\item Select most relevant AA-Methods and Hyper-parameters (Cifar-10):
\begin{todolist}
\item[\done] \textbf{ FGSM:} $\epsilon$ 2,4,8,16, iteration 1,5,10,20
\item[\done] DeepFool: iteration 1, 5, 10, 20
\item[\done] PGD: $\epsilon$ 0.1, 0.5, 1.0, 2.0, iteration 2, 3, 4, 5
\item[\done] C\&W: $c$ 0.01,0.1, 1, 5, 10 iterations 1, 10, 50, 100 \sabine{iteartion 1:useful? }
\item GenAttack: $\epsilon$ 4.0 8.0 12.0, pop\_size 6 16, iteration 50 100 150 200  \nael{ABC5x5 remaining}
\item LocalSearch: $\epsilon$ 8.0 16.0 32.0, iteration 50 100 150 200 \nael{ABC5x5 remaining}
\end{todolist}
\item Select most relevant AA-Methods and Hyper-parameters (ImageNet):
\begin{todolist}
\item FGSM: $\epsilon$  iteration 1
\item[\done] DeepFool: iteration 20
\item PGD: $\epsilon$ iteration 
\item C\&W: $c$ iterations 
\item GenAttack: $\epsilon$ 12.0 pop\_size 16 iteration 200
\item LocalSearch: $\epsilon$  iteration 
\end{todolist}
\item List of experiments, list them all:
\begin{todolist}
\item Analyze vanilla;binary;pruned)
\item[\done] new definition of hyperparameters of Attacks w.r.t. to experiment tables:
\item[\done] run experiments on ResNet20 (natural trained)
\item[\done] run experiments on ResNet20 KD (ce\_loss, kl\_loss\_20)
\item[\done] run experiments on ResNet20 XNOR
\item run experiments on ResNet20 Filterpruned
\item[\done] run experiments on ResNet20 Channelpruned
\item run experiments on ResNet20 ABC(1x1)
\item run experiments on ResNet20 ABC(3x3)
\item run experiments on ResNet20 ABC(5x5)

\item run experiments on ResNet56 (natural trained)
\item run experiments on ResNet56 XNOR
\item run experiments on ResNet56 Filterpruned, 
\item run experiments on ResNet56 Channelpruned
\item run experiments on ResNet56 ABC(1x1)
\item run experiments on ResNet56 ABC(3x3)
\item run experiments on ResNet56 ABC(5x5)

\item Analyze small to large, e.g. ResNet20, ResNet56, ResNet1xx for vanilla;binary;pruned)
\end{todolist}
\item Run CAM processor on optimized CNN and find synergies to AA
\begin{todolist}
\item[\done] ResNet20 (Vanilla, KD\_CE, KD\_KL, AMC, XNOR, ABC(1x1, 3x3, 5x5, 7x7))2 Klassen
\begin{todolist}
\item[\done] i1: Class 1 (auto) 
\item[\done] i1: Class 3 (cat)
\item[\done] i5: Class 1 (auto) 
\item[\done] i5: Class 3 (cat)

\end{todolist}

\item[\done] ResNet56 (Vanilla, AMC, XNOR, ABC(1x1, 3x3, 5x5)) - 2 Klassen
\begin{todolist}
\item[\done] i1: Class 1 (auto) 
\item[\done] i1: Class 3 (cat)
\item[\done] i5: Class 1 (auto) 
\item[\done] i5: Class 3 (cat)
\item[\done] i10 Class 1 (auto) 
\item[\done] i10: Class 3 (cat)
\end{todolist}

\item[\done] ImageNet (ResNet18, ResNet34, ResNet50, ResNet18\_XNOR, ResNet18\_AMC, ResNet34\_AMC) - 1 Klasse 751 racecar
\item[\done] ResNet18
\item[\done] ResNet18 XNOR
\item[\done] ResNet18 AMC
\item[\done] ResNet50
\end{todolist}
\end{todolist}
